Relaxed Contrastive Learning for Federated Learning

We propose a novel contrastive learning framework to effectively address the challenges of data heterogeneity in federated learning. We first analyze the inconsistency of gradient updates across clients during local training and establish its dependence on the distribution of feature representations, leading to the derivation of the supervised contrastive learning (SCL) objective to mitigate local deviations. In addition, we show that a na\"ive adoption of SCL in federated learning leads to representation collapse, resulting in slow convergence and limited performance gains. To address this issue, we introduce a relaxed contrastive learning loss that imposes a divergence penalty on excessively similar sample pairs within each class. This strategy prevents collapsed representations and enhances feature transferability, facilitating collaborative training and leading to significant performance improvements. Our framework outperforms all existing federated learning approaches by huge margins on the standard benchmarks through extensive experimental results.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
%\newcommand{\figleft}{{\em (Left)}}
%\newcommand{\figcenter}{{\em (Center)}}
%\newcommand{\figright}{{\em (Right)}}
%\newcommand{\figtop}{{\em (Top)}}
%\newcommand{\figbottom}{{\em (Bottom)}}
%\newcommand{\captiona}{{\em (a)}}
%\newcommand{\captionb}{{\em (b)}}
%\newcommand{\captionc}{{\em (c)}}
%\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
%\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
%\newcommand{\train}{\mathcal{D}}
%\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
%\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
%\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
%\def\tA{{\tens{A}}}
%\def\tB{{\tens{B}}}
%\def\tC{{\tens{C}}}
%\def\tD{{\tens{D}}}
%\def\tE{{\tens{E}}}
%\def\tF{{\tens{F}}}
%\def\tG{{\tens{G}}}
%\def\tH{{\tens{H}}}
%\def\tI{{\tens{I}}}
%\def\tJ{{\tens{J}}}
%\def\tK{{\tens{K}}}
%\def\tL{{\tens{L}}}
%\def\tM{{\tens{M}}}
%\def\tN{{\tens{N}}}
%\def\tO{{\tens{O}}}
%\def\tP{{\tens{P}}}
%\def\tQ{{\tens{Q}}}
%\def\tR{{\tens{R}}}
%\def\tS{{\tens{S}}}
%\def\tT{{\tens{T}}}
%\def\tU{{\tens{U}}}
%\def\tV{{\tens{V}}}
%\def\tW{{\tens{W}}}
%\def\tX{{\tens{X}}}
%\def\tY{{\tens{Y}}}
%\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
%\newcommand{\etens}[1]{\mathsfit{#1}}
%\def\etLambda{{\etens{\Lambda}}}
%\def\etA{{\etens{A}}}
%\def\etB{{\etens{B}}}
%\def\etC{{\etens{C}}}
%\def\etD{{\etens{D}}}
%\def\etE{{\etens{E}}}
%\def\etF{{\etens{F}}}
%\def\etG{{\etens{G}}}
%\def\etH{{\etens{H}}}
%\def\etI{{\etens{I}}}
%\def\etJ{{\etens{J}}}
%\def\etK{{\etens{K}}}
%\def\etL{{\etens{L}}}
%\def\etM{{\etens{M}}}
%\def\etN{{\etens{N}}}
%\def\etO{{\etens{O}}}
%\def\etP{{\etens{P}}}
%\def\etQ{{\etens{Q}}}
%\def\etR{{\etens{R}}}
%\def\etS{{\etens{S}}}
%\def\etT{{\etens{T}}}
%\def\etU{{\etens{U}}}
%\def\etV{{\etens{V}}}
%\def\etW{{\etens{W}}}
%\def\etX{{\etens{X}}}
%\def\etY{{\etens{Y}}}
%\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
%\newcommand{\pdata}{p_{\rm{data}}}
%% The empirical distribution defined by the training set
%\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
%\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
%% The model distribution
%\newcommand{\pmodel}{p_{\rm{model}}}
%\newcommand{\Pmodel}{P_{\rm{model}}}
%\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
%% Stochastic autoencoder distributions
%\newcommand{\pencode}{p_{\rm{encoder}}}
%\newcommand{\pdecode}{p_{\rm{decoder}}}
%\newcommand{\precons}{p_{\rm{reconstruct}}}
%
%\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution
%
%\newcommand{\E}{\mathbb{E}}
%\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\emp}{\tilde{p}}
%\newcommand{\lr}{\alpha}
%\newcommand{\reg}{\lambda}
%\newcommand{\rect}{\mathrm{rectifier}}
%\newcommand{\softmax}{\mathrm{softmax}}
%\newcommand{\sigmoid}{\sigma}
%\newcommand{\softplus}{\zeta}
%\newcommand{\KL}{D_{\mathrm{KL}}}
%\newcommand{\Var}{\mathrm{Var}}
%\newcommand{\standarderror}{\mathrm{SE}}
%\newcommand{\Cov}{\mathrm{Cov}}
%% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
%% But then they seem to use $L^2$ for vectors throughout the site, and so does
%% wikipedia.
%\newcommand{\normlzero}{L^0}
%\newcommand{\normlone}{L^1}
%\newcommand{\normltwo}{L^2}
%\newcommand{\normlp}{L^p}
%\newcommand{\normmax}{L^\infty}
%
%\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
%
%\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\Tr}{Tr}
%\let\ab\allowbreak


==> sections/umap.tex <==
% !TEX root = ../main.tex

%%%%%%%%%%%%%


%%%

\iffalse
\begin{figure*}[t]
 \centering
     %\renewcommand\thesubfigure{} % Remove subcaption numbering
    %\renewcommand\thesubfigure{(\alph{subfigure})}

    \vspace{0.cm} % Adjust vertical spacing between rows
    \begin{minipage}[t]{0.2\linewidth}
    \centering
        \caption*{Layer 1 }
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[t]{0.2\linewidth}
    \centering
        \caption*{Layer 2 }
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[t]{0.2\linewidth}
    \centering
        \caption*{Layer 3 }
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[t]{0.2\linewidth}
    \centering
        \caption*{Layer 4 }
        % \vspace{-0.2cm}
    \end{minipage}


    
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat1.png}
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat2.png}
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat3.png}
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat4.png}
    \end{minipage}
     \begin{subfigure}[t]{1\linewidth}
     \vspace{-0.5cm}
     \caption{FedAvg}
     \end{subfigure}
    \vspace{0.1cm} % Adjust vertical spacing between rows
    
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat1.png}
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat2.png}
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat3.png}
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat4.png}
    \end{minipage}

 \begin{subfigure}[t]{1\linewidth}
 \vspace{-0.2cm}
 \caption{FedGC (ours)}
 \end{subfigure}
% \vspace{0.1cm} % Adjust vertical spacing between rows

% \begin{minipage}[t]{0.2\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{./figures/L4_feat1.png}
% \end{minipage}
% \hspace{0.2cm}
% \begin{minipage}[t]{0.2\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{./figures/L4_feat2.png}
% \end{minipage}
% \hspace{0.2cm}
% \begin{minipage}[t]{0.2\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{./figures/L4_feat3.png}
% \end{minipage}
% \hspace{0.2cm}
% \begin{minipage}[t]{0.2\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{./figures/L4_feat4.png}
% \end{minipage}


%      \begin{subfigure}[t]{1\linewidth}
%      \vspace{-0.4cm}
%      \caption{FedBC-L$_4$}
%      \end{subfigure}
\vspace{0.2cm}
\caption{
% Visualization of CIFAR-100 representations: The first row showcases the case where no compatible regularization is applied (FedAvg). In the second row, the proposed method is applied to all layers.In the third row, we specifically apply the proposed method to the penultimate layer prior to the fully connected layer.
UMAP visualization of the test set of CIFAR-100 at each level, comparing (a) FedAvg baseline and (b) our full model.
% UMAP visualization of the test set of CIFAR-100 dataset at each level.
% We compared three models; (a) FedAvg baseline, (b) our full model, and (c) our ablative model FedBC-L$_4$ in Table~\ref{tab:layer_abl}.
}
\label{fig:umap}
\end{figure*}
%%%%%%%%%%%%%%%%
\fi



















\iffalse
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{./figures/base_feat0.png}
    %     \caption*{Layer 0} % Use \caption* instead of \subcaption
    %     \label{fig:figure1}
    % \end{minipage}
    % \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat1.png}
        \caption*{Layer 1}
        \label{fig:figure2}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat2.png}
        \caption*{Layer 2}
        \label{fig:figure3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat3.png}
        \caption*{Layer 3}
        \label{fig:figure4}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat4.png}
        \caption*{Layer 4}
        \label{fig:figure5}
    \end{minipage}
\caption{base}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{./figures/all_feat0.png}
    %     \caption*{Layer 0} % Use \caption* instead of \subcaption
    %     \label{fig:figure1}
    % \end{minipage}
    %\hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat1.png}
        \caption*{Layer 1}
        \label{fig:figure2}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat2.png}
        \caption*{Layer 2}
        \label{fig:figure3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat3.png}
        \caption*{Layer 3}
        \label{fig:figure4}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat4.png}
        \caption*{Layer 4}
        \label{fig:figure5}
    \end{minipage}
\caption{all}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{./figures/L4_feat0.png}
    %     \caption*{Layer 0} % Use \caption* instead of \subcaption
    %     \label{fig:figure1}
    % \end{minipage}
    %\hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat1.png}
        \caption*{Layer 1}
        \label{fig:figure2}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat2.png}
        \caption*{Layer 2}
        \label{fig:figure3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat3.png}
        \caption*{Layer 3}
        \label{fig:figure4}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat4.png}
        \caption*{Layer 4}
        \label{fig:figure5}
    \end{minipage}
\caption{L4}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{./figures/L3_feat0.png}
    %     \caption*{Layer 0} % Use \caption* instead of \subcaption
    %     \label{fig:figure1}
    % \end{minipage}
    %\hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L3_feat1.png}
        \caption*{Layer 1}
        \label{fig:figure2}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L3_feat2.png}
        \caption*{Layer 2}
        \label{fig:figure3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L3_feat3.png}
        \caption*{Layer 3}
        \label{fig:figure4}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L3_feat4.png}
        \caption*{Layer 4}
        \label{fig:figure5}
    \end{minipage}
\caption{L3}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{./figures/L2_feat0.png}
    %     \caption*{Layer 0} % Use \caption* instead of \subcaption
    %     \label{fig:figure1}
    % \end{minipage}
    %\hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L2_feat1.png}
        \caption*{Layer 1}
        \label{fig:figure2}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L2_feat2.png}
        \caption*{Layer 2}
        \label{fig:figure3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L2_feat3.png}
        \caption*{Layer 3}
        \label{fig:figure4}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L2_feat4.png}
        \caption*{Layer 4}
        \label{fig:figure5}
    \end{minipage}
\caption{L2}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{./figures/L1_feat0.png}
    %     \caption*{Layer 0} % Use \caption* instead of \subcaption
    %     \label{fig:figure1}
    % \end{minipage}
    %\hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L1_feat1.png}
        \caption*{Layer 1}
        \label{fig:figure2}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L1_feat2.png}
        \caption*{Layer 2}
        \label{fig:figure3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L1_feat3.png}
        \caption*{Layer 3}
        \label{fig:figure4}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L1_feat4.png}
        \caption*{Layer 4}
        \label{fig:figure5}
    \end{minipage}
\caption{L1}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{./figures/L0_feat0.png}
    %     \caption*{Layer 0} % Use \caption* instead of \subcaption
    %     \label{fig:figure1}
    % \end{minipage}
    % \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L0_feat1.png}
        \caption*{Layer 1}
        \label{fig:figure2}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L0_feat2.png}
        \caption*{Layer 2}
        \label{fig:figure3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L0_feat3.png}
        \caption*{Layer 3}
        \label{fig:figure4}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L0_feat4.png}
        \caption*{Layer 4}
        \label{fig:figure5}
    \end{minipage}
\caption{L0}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    \captionsetup[subfigure]{labelformat=empty} % Remove subfigure labels
    
    % Row: all
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat0.png}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat1.png}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat2.png}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat3.png}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat4.png}
    \end{minipage}

    \vspace{1cm} % Add vertical space between the rows
    
    % Row: L4
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat0.png}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat1.png}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat2.png}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat3.png}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat4.png}
    \end{minipage}
    
    \caption{Caption for the entire figure}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    
    % Row: all
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat0.png}
        \caption*{Layer 0}
        \label{fig:all_feat0}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat1.png}
        \caption*{Layer 1}
        \label{fig:all_feat1}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat2.png}
        \caption*{Layer 2}
        \label{fig:all_feat2}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat3.png}
        \caption*{Layer 3}
        \label{fig:all_feat3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat4.png}
        \caption*{Layer 4}
        \label{fig:all_feat4}
    \end{minipage}
    
    \vspace{1cm} % Add vertical space between the rows
    
    % Row: L4
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat0.png}
        \caption*{Layer 0}
        \label{fig:L4_feat0}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat1.png}
        \caption*{Layer 1}
        \label{fig:L4_feat1}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat2.png}
        \caption*{Layer 2}
        \label{fig:L4_feat2}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat3.png}
        \caption*{Layer 3}
        \label{fig:L4_feat3}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat4.png}
            \caption*{Layer 4}
        \label{fig:all_feat4}
    \end{minipage}
\end{figure*}
\fi




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \renewcommand\thesubfigure{} % Remove subcaption numbering
    
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat1.png}
        \caption*{Layer 1 (Base)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat2.png}
        \caption*{Layer 2 (Base)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat3.png}
        \caption*{Layer 3 (Base)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/base_feat4.png}
        \caption*{Layer 4 (Base)}
    \end{minipage}

    \vspace{0.5cm} % Adjust vertical spacing between rows
    
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat1.png}
        \caption*{Layer 1 (All)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat2.png}
        \caption*{Layer 2 (All)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat3.png}
        \caption*{Layer 3 (All)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/all_feat4.png}
        \caption*{Layer 4 (All)}
    \end{minipage}

    \vspace{0.5cm} % Adjust vertical spacing between rows
    
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat1.png}
        \caption*{Layer 1 (L4)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat2.png}
        \caption*{Layer 2 (L4)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figures/L4_feat3.png}
        \caption*{Layer 3 (L4)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
\centering
\includegraphics[width=\linewidth]{./figures/L4_feat4.png}
\caption*{Layer 4 (L4)}
\end{minipage}

\caption{Comparison of metric loss at different layers}
\end{figure*}
\fi


\begin{figure*}
    \centering
    % \begin{subfigure}{0.18\textwidth}
    %     \includegraphics[width=\linewidth]{./figures/umap_fedavg0.05.pdf}
    %     \caption{FedAvg}
    % \end{subfigure}
    \begin{subfigure}{0.16\textwidth}
        \includegraphics[width=\linewidth]{./figures/umap_proc005.pdf}
        \caption{FedProc}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.16\textwidth}
        \includegraphics[width=\linewidth]{./figures/umap_lc005.pdf}
        \caption{FedLC}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.16\textwidth}
        \includegraphics[width=\linewidth]{./figures/umap_decorr005.pdf}
        \caption{FedDecorr}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.16\textwidth}
        \includegraphics[width=\linewidth]{./figures/umap_rcl005.pdf}
        \caption{FedRCL (ours)}
    \end{subfigure}
    \caption{UMAP Visualization of the extracted features from the global model under severe data heterogeneity.}
    \label{fig:umap}
\end{figure*}




% \begin{figure*}
%     \centering
%     % \begin{subfigure}{0.18\textwidth}
%     %     \includegraphics[width=\linewidth]{./figures/umap_fedavg0.05.pdf}
%     %     \caption{FedAvg}
%     % \end{subfigure}
%     \begin{subfigure}{0.16\textwidth}
%         \includegraphics[width=\linewidth]{./figures/umap_proc.pdf}
%         \caption{FedProc}
%     \end{subfigure}
%     \hspace{0.5cm}
%     \begin{subfigure}{0.16\textwidth}
%         \includegraphics[width=\linewidth]{./figures/umap_lc.pdf}
%         \caption{FedLC}
%     \end{subfigure}
%     \hspace{0.5cm}
%     \begin{subfigure}{0.16\textwidth}
%         \includegraphics[width=\linewidth]{./figures/umap_decorr.pdf}
%         \caption{FedDecorr}
%     \end{subfigure}
%     \hspace{0.5cm}
%     \begin{subfigure}{0.16\textwidth}
%         \includegraphics[width=\linewidth]{./figures/umap_rcl.pdf}
%         \caption{FedRCL (ours)}
%     \end{subfigure}
%     \caption{UMAP Visualization of the extracted features from the global model under severe data heterogeneity.}
%     \label{fig:umap}
% \end{figure*}
